Continual Detection Transformer for Incremental Object Detection

Incremental object detection (IOD) aims to train an object detector in phases, each with annotations for new object categories. As other incremental settings, IOD is subject to catastrophic forgetting, which is often addressed by techniques such as knowledge distillation (KD) and exemplar replay (ER). However, KD and ER do not work well if applied directly to state-of-the-art transformer-based object detectors such as Deformable DETR and UP-DETR. In this paper, we solve these issues by proposing a ContinuaL DEtection TRansformer (CL-DETR), a new method for transformer-based IOD which enables effective usage of KD and ER in this context. First, we introduce a Detector Knowledge Distillation (DKD) loss, focusing on the most informative and reliable predictions from old versions of the model, ignoring redundant background predictions, and ensuring compatibility with the available ground-truth labels. We also improve ER by proposing a calibration strategy to preserve the label distribution of the training set, therefore better matching training and testing statistics. We conduct extensive experiments on COCO 2017 and demonstrate that CL-DETR achieves state-of-the-art results in the IOD setting.

==> tables/table_ablation_backup.tex <==
\begin{table*}
\small
\centering
\setlength{\tabcolsep}{1.45mm}{
\begin{tabular}{@{}llcccccccccccccccc@{}}
\toprule
  \multirow{2.5}{*}{\textbf{No.}} & \multirow{2.5}{*}{\textbf{Setting}} & \multicolumn{4}{c}{All categories $\uparrow$}  && \multicolumn{4}{c}{Old categories $\uparrow$} && \multicolumn{4}{c}{Forgetting $\downarrow$}\\
  \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16}
     &  & $AP$ & $AP_{S}$  & $AP_{M}$  & $AP_{L}$ && $AP$ & $AP_{S}$  & $AP_{M}$  & $AP_{L}$ && $AP$ &$AP_{S}$  & $AP_{M}$  & $AP_{L}$\\
    \midrule
    1&Finetuning & 4.2 & 1.6  & 4.7 &5.8 && 0.7 & 0.2 & 0.8 & 0.8 && 42.6 & 25.6 & 45.1 & 56.7    \\%\\ 
    2&Ours & 39.7 & 20.9  & 40.8 & 50.7 && 41.1 &24.2 &43.6 & 54.0 && 2.2 & 1.6 & 2.3 & 3.5\\%\\ 
   \midrule
     3&\emph{w/o} Pseudo label selection  & 30.3 & 19.5  & 33.0 & 39.0 && 33.4 & 21.8 & 36.4 & 43.2 && 9.9 &4.0 & 9.5 & 14.3 \\
    4&\emph{w/o} Joint bipartite matching  & 35.9 & 19.1  & 39.4 & 48.6 && 36.8 & 20.3 & 39.9 & 50.0 && 6.5 & 5.5 & 6.0 &7.5  \\
     5&\emph{w/o} Distribution preserved calibration & 33.9 & 16.3  & 37.1 & 49.2 && 33.9  & 16.6 & 36.8 & 50.0 && 9.4 & 9.2 & 9.1 & 7.5\\
\bottomrule     
\end{tabular}
}
\caption{Ablation results (\%) on COCO 2017 using the $70+10$ setup. ``All categories'' (higher is better) denotes the results of $\theta_2$ on $80$ categories. ``Old categories'' (higher is better) denotes the results of $\theta_2$ on $70$ categories observed in the $1$-st phase. ``Forgetting'' (lower is better) shows the difference between the AP of $\theta_1$ and $\theta_2$ on $70$ categories observed in the $1$-st phase.}
\label{table_ablation_1}
\vspace{-0.8em}
\end{table*}

==> tables/table_sota_backup.tex <==
\begin{table*}
\small
\centering
\setlength{\tabcolsep}{3.25mm}{
\begin{tabular}{l|lcccccccc}
\toprule
Setup    & Method & Detection baseline & $AP$ & $AP_{50}$ & $AP_{75}$  & $AP_{S}$  & $AP_{M}$  & $AP_{L}$  \\ \midrule
  \multirow{9}{*}{$70$+$10$} & LwF$^*$ \cite{LiH2018LwF} & GFLv1   & 7.1  & 12.4  & 7.0 & 4.8  & 9.5 & 10.0\\
    & RILOD$^*$ \cite{Li2019RILOD} & GFLv1   & 24.5 & 37.9  & 25.7 & 14.2  & 27.4 & 33.5\\
    & SID$^*$ \cite{Peng2021SID} & GFLv1   & 32.8  & 49.0  & 35.0 & 17.1  & 36.9 & 44.5\\
    & ERD$^*$ \cite{Feng2022ElasticResponse}  & GFLv1   & {34.9 } & {51.9}  & {37.4}  & {18.7}  & {38.8}   & {45.5}\\
    \cmidrule(l){2-9}
     & LwF \cite{LiH2018LwF} & Deformable DETR   & 24.5 & 36.6  & 26.7 & 12.4  & 28.2 & 35.2 \\
     & iCaRL \cite{Rebuffi2017iCaRL} & Deformable DETR   & 35.9 & 52.5  & 39.2 & 19.1  & 39.4 & 48.6 \\
     & ERD \cite{Feng2022ElasticResponse} & Deformable DETR    & 36.2 & 54.8  & 39.3 & 20.8  & 39.3 & 47.9 \\
     & \cellcolor{mygray-bg}{CL-DETR (ours)} & \cellcolor{mygray-bg}{UP-DETR}  &  \cellcolor{mygray-bg}{{37.6}\tiny{$\pm$0.2}} & \cellcolor{mygray-bg}{{56.5}\tiny{$\pm$0.4}}  & \cellcolor{mygray-bg}{{39.4}\tiny{$\pm$0.3}} & \cellcolor{mygray-bg}{{20.5}\tiny{$\pm$0.3}}  & \cellcolor{mygray-bg}{{39.1}\tiny{$\pm$0.4}} & \cellcolor{mygray-bg}{{49.9}\tiny{$\pm$0.3}} \\
     & \cellcolor{mygray-bg}{CL-DETR (ours)} & \cellcolor{mygray-bg}{Deformable DETR} &  \cellcolor{mygray-bg}{\textbf{39.7}\tiny{$\pm$0.4}} & \cellcolor{mygray-bg}{\textbf{57.4}\tiny{$\pm$0.4}}  & \cellcolor{mygray-bg}{\textbf{43.1}\tiny{$\pm$0.3}} & \cellcolor{mygray-bg}{\textbf{22.7}\tiny{$\pm$0.4}}  & \cellcolor{mygray-bg}{\textbf{42.6}\tiny{$\pm$0.3}} & \cellcolor{mygray-bg}{\textbf{52.7}\tiny{$\pm$0.3}} \\
     \\[-12pt]
     \midrule
   \multirow{9}{*}{$40$+$40$} & LwF$^*$ \cite{LiH2018LwF} & GFLv1   & 17.2  & 25.4  & 18.6 & 7.9  & 18.4 & 24.3\\
    & RILOD$^*$ \cite{Li2019RILOD} & GFLv1   & 29.9  & 45.0  & 32.0 & 15.8  & 33.0 & 40.5\\
    & SID$^*$ \cite{Peng2021SID} & GFLv1   & 34.0  & 51.4  & 36.3 & 18.4  & 38.4 & 44.9\\
    & ERD$^*$ \cite{Feng2022ElasticResponse} & GFLv1   & {36.9} & {54.5}  & {39.6}  & {21.3}  & {40.4}   & {47.5}\\ 
    \cmidrule(l){2-9}
     & LwF \cite{LiH2018LwF} & Deformable DETR   & -- & --  & -- & --  & -- & -- \\
     & iCaRL \cite{Rebuffi2017iCaRL} & Deformable DETR   & -- & --  & -- & --  & -- & -- \\
     & ERD \cite{Feng2022ElasticResponse} & Deformable DETR   & -- & --  & -- & --  & -- & -- \\
     & \cellcolor{mygray-bg}{CL-DETR (ours)} & \cellcolor{mygray-bg}{UP-DETR}  &  \cellcolor{mygray-bg}{{37.0}\tiny{$\pm$0.2}} & \cellcolor{mygray-bg}{{56.2}\tiny{$\pm$0.2}}  & \cellcolor{mygray-bg}{{39.1}\tiny{$\pm$0.4}} & \cellcolor{mygray-bg}{{20.9}\tiny{$\pm$0.2}}  & \cellcolor{mygray-bg}{{38.9}\tiny{$\pm$0.3}} & \cellcolor{mygray-bg}{{49.2}\tiny{$\pm$0.3}} \\
     & \cellcolor{mygray-bg}{CL-DETR (ours)} & \cellcolor{mygray-bg}{Deformable DETR} &  \cellcolor{mygray-bg}{\textbf{37.5}\tiny{$\pm$0.3}} & \cellcolor{mygray-bg}{\textbf{55.1}\tiny{$\pm$0.4}}  & \cellcolor{mygray-bg}{\textbf{40.3}\tiny{$\pm$0.2}} & \cellcolor{mygray-bg}{{20.9}\tiny{$\pm$0.2}}  & \cellcolor{mygray-bg}{\textbf{40.8}\tiny{$\pm$0.4}} & \cellcolor{mygray-bg}{\textbf{50.7}\tiny{$\pm$0.2}} \\
     [-2pt]
\bottomrule 
\multicolumn{9}{l}{$^*$ The results are from~\cite{Feng2022ElasticResponse} and use more training samples than our benchmark protocol.}\\
\multicolumn{9}{l}{\textcolor[rgb]{1,1,1}{$^*$} We also provide the results of our method using \cite{Feng2022ElasticResponse}'s baseline protocol in the supplementary. }
\end{tabular}
}
\caption{IOD results (\%) on COCO 2017 in the following setups. \emph{\textbf{(1) ``40+40''.}}  In the $1$-st phase, we observe half of the training samples with $40$ categories annotated. In the $2$-nd phase, we observe the other half of the training samples, where $40$ new categories are annotated. \emph{\textbf{(2) ``70+10''.}} In the $1$-st phase, we observe $\frac{7}{8}$ of the training samples with $70$ categories annotated. In the $2$-nd phase, we observe the remaining $\frac{1}{8}$ of the training samples, where $10$ new categories are annotated. For the experiments on Deformable DETR~\cite{Zhu2021DeformableDETR} and UP-DETR~\cite{Dai2021UPDETR}, we run experiments for three different categories and data orders and report the average AP. For the experiments on GFLv1~\cite{Li2020GFL}, we use the results from~\cite{Feng2022ElasticResponse}. }
\label{table_sota}
\vspace{-0.8em}
\end{table*}
